Inverse optimal control problem in the non autonomous linear-quadratic case

Inverse optimal control problem emerges in different practical applications, where the goal is to design a cost function in order to approximate given optimal strategies of an expert. Typical application is in robotics for generation of human motions. In this paper we analyze a general class of non autonomous inverse linear quadratic problems. This class of problems is of particular interest because it arises as a linearization of a nonlinear problem around an optimal trajectory. The addressed questions are the injectivity of the inverse problem and the reconstruction. We show that the nonlinear problem admits the same characterization of the injectivity as the autonomous one. In the autonomous case we show moreover that the injectivity property is generic in the considered class. We also provide a numerical test of the reconstruction algorithm in the autonomous setting.

==> Biblio/biblio_LQ.tex <==
@Article{Jurdjevic1989,
  author =    {Jurdjevic, V and Kogan, J},
  title =     {Optimality of extremals for linear systems with quadratic costs},
  journal =   {Journal of Mathematical Analysis and Applications},
  year =      {1989},
  volume =    {143},
  pages =     {86-108},
  month =     {10},
  doi =       {10.1016/0022-247X(89)90030-9},
  file =      {:Optimal_control\\jurdjevic1989.pdf:PDF},
  keywords =  {2nd order, optimal control, linear control, quadratic cost},
  owner =     {Frédéric Jean},
  timestamp = {28.11.2018}
}

@Article{Brunovsky1981,
  author =    {P. Brunovsky and J. Komornik},
  title =     {The Riccati equation solution of the linear-quadratic problem with constrained terminal state},
  journal =   {IEEE Transactions on Automatic Control},
  year =      {1981},
  volume =    {26},
  number =    {2},
  pages =     {398-402},
  month =     {April},
  doi =       {10.1109/TAC.1981.1102600},
  file =      {:Optimal_control\\brunovsky1981.pdf:PDF},
  issn =      {0018-9286},
  keywords =  {Algebraic Riccati equation (ARE);Linear-quadratic control;Riccati equations, algebraic;Riccati equations;Closed-form solution;Automatic control;Controllability;Optimal control;State feedback;Sufficient conditions;Kalman filters;Temperature control, linear control, quadratic cost, optimal control},
  owner =     {Frédéric Jean},
  timestamp = {16.11.2018}
}

@Article{Molinari1977,
  author    = {B.P. Molinari},
  journal   = {Automatica},
  title     = {The time-invariant linear-quadratic optimal control problem},
  year      = {1977},
  issn      = {0005-1098},
  number    = {4},
  pages     = {347 - 357},
  volume    = {13},
  doi       = {http://dx.doi.org/10.1016/0005-1098(77)90017-6},
  file      = {:Optimal_control\\molinari77.pdf:PDF},
  keywords  = {Optimal control, linear control, optimal control},
  owner     = {Frédéric Jean},
  timestamp = {01.05.2016},
  url       = {http://www.sciencedirect.com/science/article/pii/0005109877900176},
}

@BOOK{Jurdjevic1996,
  title = {Geometric Control Theory},
  publisher = {Cambridge University Press},
  year = {1996},
  author = {V. Jurdjevic},
  file = {:Livres/Djvu/Jurdjevic_Geometric_Control_Theory__1996.djvu:Djvu},
  keywords = {geometric control, control-affine, optimal control},
  owner = {Frédéric Jean},
  timestamp = {18.10.2012}
}

@BOOK{Schaettler2012,
  title = {Geometric Optimal Control},
  publisher = {Springer},
  year = {2012},
  author = {H. Sch\"{a}ttler and U. Ledzewicz},
  file = {:Livres/Schattler_Ledzewicz_-Geometric_optimal_control_theory,_methods_and_examples-Springer(2012).pdf:PDF},
  keywords = {geometric control, optimal control},
  owner = {Frédéric Jean},
  timestamp = {28.01.2013}
}

@Article{Mereau1976,
  author =     {Mereau, P. M. and Powers, W. F.},
  title =      {Conjugate point properties for linear quadratic problems},
  journal =    {J. Math. Anal. Appl.},
  year =       {1976},
  volume =     {55},
  number =     {2},
  pages =      {418--433},
  doi =        {10.1016/0022-247X(76)90172-4},
  file =       {:Optimal_control\\mereau_powers76.pdf:PDF},
  fjournal =   {Journal of Mathematical Analysis and Applications},
  issn =       {0022-247x},
  keywords =   {2nd order, linear control, quadratic cost},
  mrclass =    {49D30 (93C05)},
  mrnumber =   {0454820},
  mrreviewer = {D. F. Lawden},
  owner =      {Frédéric Jean},
  timestamp =  {27.11.2018},
  url =        {https://doi.org/10.1016/0022-247X(76)90172-4}
}

@Book{Agrachev2004,
  author    = {A. A. Agrachev and Y. L. Sachkov},
  publisher = {Springer-Verlag},
  title     = {Control Theory from the Geometric Viewpoint},
  year      = {2004},
  file      = {:Livres\\Djvu\\Agrachev_Sachkov,_Andrei_Agrachev.djvu:Djvu},
  keywords  = {geometric control, optimal control, SR geometry},
  owner     = {Fr\'{e}d\'{e}ric Jean},
  timestamp = {10.02.2007},
}

@Article{Li2020,
  author   = {Yibei Li and Yu Yao and Xiaoming Hu},
  journal  = {Automatica},
  title    = {Continuous-time inverse quadratic optimal control problem},
  year     = {2020},
  issn     = {0005-1098},
  pages    = {108977},
  volume   = {117},
  abstract = {In this paper, the problem of finite horizon inverse optimal control (IOC) is investigated, where the quadratic cost function of a dynamic process is required to be recovered based on the observation of optimal control sequences. We propose the first complete result of the necessary and sufficient condition for the existence of corresponding standard linear quadratic (LQ) cost functions. Under feasible cases, the analytic expression of the whole solution space is derived and the equivalence of weighting matrices in LQ problems is discussed. For infeasible problems, an infinite dimensional convex problem is formulated to obtain a best-fit approximate solution with minimal control residual. And the optimality condition is solved under a static quadratic programming framework to facilitate the computation. Finally, numerical simulations are used to demonstrate the effectiveness and feasibility of the proposed methods.},
  doi      = {https://doi.org/10.1016/j.automatica.2020.108977},
  file     = {:Inverse/Li2020.pdf:PDF},
  keywords = {Inverse dynamic problem, Linear quadratic regulators, Optimal control, Linear matrix inequality, inverse problem, optimal control, quadratic cost, linear control},
  url      = {https://www.sciencedirect.com/science/article/pii/S0005109820301758},
}

Scopus
EXPORT DATE: 5 November 2021

@Article{Li20211840,
  author        = {Li, Y. and Wahlberg, B. and Hu, X.},
  journal       = {Journal of Systems Science and Complexity},
  title         = {Identifiability and Solvability in Inverse Linear Quadratic Optimal Control Problems},
  year          = {2021},
  note          = {cited By 0},
  number        = {5},
  pages         = {1840-1857},
  volume        = {34},
  document_type = {Article},
  doi           = {10.1007/s11424-021-1245-3},
  file          = {:Inverse/Li2021_Article_IdentifiabilityAndSolvabilityI.pdf:PDF},
  keywords      = {inverse problem, quadratic cost, linear control},
  source        = {Scopus},
  url           = {https://www.scopus.com/inward/record.uri?eid=2-s2.0-85117961728&doi=10.1007%2fs11424-021-1245-3&partnerID=40&md5=a1b7414432a7b4423ba46b1a949ff320},
}

@Book{Kwakernaak1972,
  author     = {Kwakernaak, Huibert and Sivan, Raphael},
  publisher  = {Wiley-Interscience [John Wiley \& Sons], New York-London-Sydney},
  title      = {Linear optimal control systems},
  year       = {1972},
  file       = {:Livres/kwakernaak-linear-optimal-control-systems.pdf:PDF},
  keywords   = {linear control, optimal control},
  mrclass    = {93C05},
  mrnumber   = {0406607},
  mrreviewer = {Takashi Yahagi},
  pages      = {xxv+575},
}

@Book{AbouKandil2003,
  author    = {Hisham Abou-Kandil and Gerhard Freiling and Vlad Ionescu and Gerhard Jank},
  publisher = {Birkh\"{a}user Basel},
  title     = {Matrix Riccati Equations in Control and Systems Theory},
  year      = {2003},
  doi       = {10.1007/978-3-0348-8081-7},
  file      = {:Livres/Abou-Kandil2003_Book_MatrixRiccatiEquationsInContro.pdf:PDF},
  keywords  = {quadratic cost, linear control, optimal control},
  url       = {https://doi.org/10.1007/978-3-0348-8081-7},
}

@Article{Todorov2002,
  author  = {E. Todorov, and M. I. Jordan},
  title   = {Optimal feedback control as a theory of motor coordination},
  journal = {Nat Neurosci},
  year    = {2002},
  volume  = {5},
  pages   = {1226-1235},
}

@InProceedings{Todorov2006,
  author    = {E. Todorov},
  title     = {Optimal control theory},
  booktitle = {Bayesian Brain: Probabilistic Approaches to Neural Coding},
  year      = {2006},
  editor    = {Doya K.},
  pages     = {269-298},
  chapter   = {12},
}

@Article{Arechavaleta2008,
  author  = {Arechavaleta, Gustavo and Laumond, Jean-Paul and Hicheur, Halim and Berthoz, Alain},
  journal = {IEEE Transactions on Robotics},
  title   = {An Optimality Principle Governing Human Walking},
  year    = {2008},
  number  = {1},
  pages   = {5-14},
  volume  = {24},
  doi     = {10.1109/TRO.2008.915449},
}

@Article{Nielsen2004,
  author  = {T. Nielsen and F. Jensen},
  title   = {Learning a decision maker's utility function from (possibly) inconsistent behavior},
  journal = {Artificial Intelligence},
  year    = {2004},
  volume  = {160},
  pages   = {53-78},
}

@TechReport{Anderson1966,
  author  = {Anderson, B.D.O.},
  title   = {The Inverse Problem of Linear Optimal Control},
  year    = {1966},
  address = {CA},
  number  = {SEL-66-039},
  type    = {techreport},
  school  = {Stanford University},
}

@Article{Kalman1964,
  author    = {Kalman, R. E.},
  title     = {When Is a Linear Control System Optimal?},
  journal   = {Journal of Basic Engineering},
  year      = {1964},
  volume    = {86},
  number    = {1},
  pages     = {51--60},
  month     = mar,
  issn      = {0098-2202},
  abstract  = {The purpose of this paper is to formulate, study, and (in certain cases) resolve the Inverse Problem of Optimal Control Theory, which is the following: Given a control law, find all performance indices for which this control law is optimal. Under the assumptions of (a) linear constant plant, (b) linear constant control law, (c) measurable state variables, (d) quadratic loss functions with constant coefficients, (e) single control variable, we give a complete analysis of this problem and obtain various explicit conditions for the optimality of a given control law. An interesting feature of the analysis is the central role of frequency-domain concepts, which have been ignored in optimal control theory until very recently. The discussion is presented in rigorous mathematical form. The central conclusion is the following (Theorem 6): A stable control law is optimal if and only if the absolute value of the corresponding return difference is at least equal to one at all frequencies. This provides a beautifully simple connecting link between modern control theory and the classical point of view which regards feedback as a means of reducing component variations.},
  comment   = {10.1115/1.3653115},
  doi       = {10.1115/1.3653115},
  publisher = {ASME},
  url       = {http://dx.doi.org/10.1115/1.3653115},
}

@Article{Kreindler1970,
  author    = {Eliezer Kreindler and J. Karl Hedrick},
  journal   = {International Journal of Control},
  title     = {On equivalence of quadratic loss functions},
  year      = {1970},
  number    = {2},
  pages     = {213-222},
  volume    = {11},
  abstract  = {When a linear, time.invariant plant is optimized with respect to the performance index where x is the state vector and u the control, the optimal control can be expressed as a feedback law u = –Kx Two pairs of matrices [Q, R] and [Q e, R e], yielding the same control law are equivalent. A necessary and sufficient condition is derived, in the single–input case, for a symmetric non–negative definite Q to be equivalent to a diagonal matrix Q*. This condition is satisfied by a plant described by equations in phase–variable canonical form, and a formula for Q* in terms of Q is given. It is shown that an equivalent Q e can be parameterized by exactly n non–negative parameters. For the multi–input case, Q e and R e must contain at least nr parameters, where n and r are the dimensions of x and u, respectively.},
  doi       = {10.1080/00207177008905900},
  eprint    = {https://doi.org/10.1080/00207177008905900},
  publisher = {Taylor \& Francis},
  url       = {https://doi.org/10.1080/00207177008905900},
}

@Article{Kreindler1972,
  author   = {E. Kreindler and A. Jameson},
  title    = {Optimality of linear control systems},
  journal  = {IEEE Transactions on Automatic Control},
  year     = {1972},
  volume   = {17},
  number   = {3},
  pages    = {349-351},
  month    = {Jun},
  issn     = {0018-9286},
  abstract = {It is shown that every linear system with nondynamic feedback is optimal with respect to a quadratic performance index that includes a cross-product term between the state and control. If the index is further generalized to include derivatives of the control, every (sufficiently smooth) linear finite-dimensional dynamic feedback and feedforward control system is optimal. Methods of constructing all such indices are indicated, and some practical implications are discussed.},
  doi      = {10.1109/TAC.1972.1099985},
  keywords = {Inverse optimal control problem;Linear systems, time-varying continuous-time;Control systems;Eigenvalues and eigenfunctions;Equations;Matrices;Optimal control;Optimization methods},
}

@Book{Zenkov2015,
  title     = {The inverse problem of the calculus of variations. Local and global theory.},
  publisher = {Atlantis Press},
  year      = {2015},
  editor    = {Dmitry V. Zenkov},
  series    = {2},
  isbn      = {978-94-6239-108-6},
}

@Article{Anderson1992,
  author  = {Anderson, I. M., and Thompson, J.},
  title   = {The Inverse problem of the calculus of variations for ordinary differential equations},
  journal = {Memoirs of the American Mathematical Society},
  year    = {1992},
  volume  = {98},
}

@Article{Sonin1886,
  author  = {Sonin, N.Ya.},
  title   = {On determining maximal and minimal properties of planar curves},
  journal = {Varshavskie Universitetskie Izvestiya, Russian},
  year    = {1886},
  number  = {1-2},
  pages   = {1-68},
  note    = {English transpation: Lepage Research Institute. Archive no. 1 (2012)},
}

@Article{Helmholtz1887,
  author  = {Helmholtz, H.},
  title   = {Uber die physikalische Bedeutung des Prinzips der kleinsten Wirkung},
  journal = {J. fur die Reine Angewandte Math.},
  year    = {1887},
  volume  = {100},
  pages   = {137-166},
  url     = {https://ci.nii.ac.jp/naid/10011581454/en/},
}

@Article{Mayer1896,
  author  = {Mayer, Adolph},
  title   = {Die Existenz bedingungen eines kinetischen Potentiales},
  journal = {Berich. Verh. Konig. Sach. Gesell. wissen. Leipzig, Math. Phys. Kl.},
  year    = {1896},
  volume  = {84},
  pages   = {519-529},
}

@Article{Saunders2010,
  author   = {D.J. Saunders},
  title    = {Thirty years of the inverse problem in the calculus of variations},
  journal  = {Reports on Mathematical Physics},
  year     = {2010},
  volume   = {66},
  number   = {1},
  pages    = {43-53},
  issn     = {0034-4877},
  abstract = {We consider several aspects of the inverse problem of the calculus of variations as they have developed since 1979, giving some of the principal results, listing significant primary sources and mentioning review articles for further references. The main topics involve questions of the existence and uniqueness of a Lagrangian giving rise to a given family of differential equations; we also describe some different types of inverse problem which arise in the context of quantum mechanics.},
  doi      = {https://doi.org/10.1016/S0034-4877(10)00022-4},
  keywords = {inverse problem, calculus of variations},
  url      = {http://www.sciencedirect.com/science/article/pii/S0034487710000224},
}

@Article{Douglas1941,
  author    = {Douglas, Jesse},
  title     = {Solution of the Inverse Problem of the Calculus of Variations},
  journal   = {Transactions of the American Mathematical Society},
  year      = {1941},
  volume    = {50},
  number    = {1},
  pages     = {71--128},
  issn      = {00029947},
  publisher = {American Mathematical Society},
  url       = {http://www.jstor.org/stable/1989912},
}

@Article{Anderson1980,
  author    = {Anderson, I. M. and Duchamp, T.},
  title     = {On the Existence of Global Variational Principles},
  journal   = {American Journal of Mathematics},
  year      = {1980},
  volume    = {102},
  number    = {5},
  pages     = {781--868},
  issn      = {00029327, 10806377},
  publisher = {Johns Hopkins University Press},
  url       = {http://www.jstor.org/stable/2374195},
}

@Article{Krupkova1997,
  author    = {Krupkov{\'a}, Olga},
  title     = {The Geometry of Ordinary Variational Equations},
  journal   = {Lecture notes in Mathematics},
  year      = {1997},
  volume    = {1678},
  address   = {Berlin},
  publisher = {Springer},
}

@Book{Volterra1913,
  title     = {Le{\c{c}}ons sur les fonctions de lignes, profess{\'e}es {\`a} la Sorbonne en 1912, par Vito Volterra,... recueillies et r{\'e}dig{\'e}es par Joseph P{\'e}r{\`e}s,...},
  publisher = {Gauthier-Villars},
  year      = {1913},
  author    = {Volterra, Vito},
}

@Book{Vainberg1959,
  title     = {Variational Methods for the Study of Nonlinear Operators},
  publisher = {Holden-Day},
  year      = {1964},
  author    = {M.M. Vainberg},
  address   = {San Francisco},
  note      = {Transl. from Russian (GITL, Moscow, 1959)},
}

@Article{Tonti1969,
  author  = {E. Tonti},
  title   = {Variational formulation of nonlinear differential equations I, II,},
  journal = {Bulletin de la Classe des Sciences, Acad\'{e}mie royale de Belgique},
  year    = {1969},
  volume  = {55},
  number  = {4},
  pages   = {137-165, 262-278},
}

@Article{Fujii1984,
  author  = {Fujii, T. and Narazaki, M.},
  journal = {SIAM Journal on Control and Optimization},
  title   = {A Complete Optimality Condition in the Inverse Problem of Optimal Control},
  year    = {1984},
  number  = {2},
  pages   = {327-341},
  volume  = {22},
  doi     = {10.1137/0322022},
  eprint  = {https://doi.org/10.1137/0322022},
  url     = {https://doi.org/10.1137/0322022},
}

@Article{Yamamoto1987,
  author    = {Kenji Sugimoto and Yutaka Yamamoto},
  journal   = {International Journal of Control},
  title     = {New solution to the inverse regulator problem by the polynomial matrix method},
  year      = {1987},
  number    = {5},
  pages     = {1627-1640},
  volume    = {45},
  abstract  = {Abstract This paper gives a new criterion for the inverse regulator problem in terms of polynomial matrix fractions. The generalized Kalman equation in polynomial matrix form leads to a necessary and sufficient condition for a stable feedback law to be optimal for some (unknown) quadratic performance index. This criterion consists of (i) a symmetric factorizability of a polynomial matrix, and (ii) a polynomial-type criterion that guarantees detectability. The relationship between the Riccati and Kalman equations is also established. Finally, an example is given to illustrate the new result in contrast with the existing result.},
  doi       = {10.1080/00207178708933838},
  eprint    = {https://doi.org/10.1080/00207178708933838},
  publisher = {Taylor \& Francis},
  url       = {https://doi.org/10.1080/00207178708933838},
}

@InProceedings{Pauwels2014,
  author    = {Pauwels, Edouard and Henrion, Didier and Lasserre, Jean-Bernard},
  booktitle = {53rd IEEE Conference on Decision and Control},
  title     = {Inverse optimal control with polynomial optimization},
  year      = {2014},
  pages     = {5581-5586},
  doi       = {10.1109/CDC.2014.7040262},
}

@Article{Ajami2013,
  author    = {Ajami, Alain and Gauthier, Jean-Paul and Maillot, Thibault and Serres, Ulysse},
  title     = {How humans fly},
  journal   = {ESAIM: Control, Optimisation and Calculus of Variations},
  year      = {2013},
  volume    = {19},
  number    = {4},
  pages     = {1030-1054},
  issn      = {1292-8119},
  abstract  = {This paper is devoted to the general problem of reconstructing the cost from the          observation of trajectories, in a problem of optimal control. It is motivated by the          following applied problem, concerning HALE drones: one would like them to decide by          themselves for their trajectories, and to behave at least as a good human pilot. This          applied question is very similar to the problem of determining what is minimized in human          locomotion. These starting points are the reasons for the particular classes of control          systems and of costs under consideration. To summarize, our conclusion is that in general,          inside these classes, three experiments visiting the same values of the control are needed          to reconstruct the cost, and two experiments are in general not enough. The method is          constructive. The proof of these results is mostly based upon the Thom’s transversality theory. This study is partly supported by FUI AAP9 project SHARE, and by ANR Project GCM, program          “blanche”, project number NT09-504490.},
  database  = {Cambridge Core},
  doi       = {10.1051/cocv/2012043},
  edition   = {2013/06/03},
  keywords  = {Inverse optimal control, anthropomorphic control, transversality},
  publisher = {EDP Sciences},
  url       = {https://www.cambridge.org/core/article/how-humans-fly/CB7474A51520946D513F28F7087A349F},
}

@InProceedings{Kuderer2015,
  author    = {Kuderer, M. and Gulati, S. and Burgard, W.},
  title     = {Learning driving styles for autonomous vehicles from demonstration},
  booktitle = {IEEE International Conference on Robotics and Automation (ICRA)},
  year      = {2015},
  pages     = {2641--2646},
  abstract  = {It is expected that autonomous vehicles capable of driving without human supervision will be released to market within the next decade. For user acceptance, such vehicles should not only be safe and reliable, they should also provide a comfortable user experience. However, individual perception of comfort may vary considerably among users. Whereas some users might prefer sporty driving with high accelerations, others might prefer a more relaxed style. Typically, a large number of parameters such as acceleration profiles, distances to other cars, speed during lane changes, etc., characterize a human driver's style. Manual tuning of these parameters may be a tedious and error-prone task. Therefore, we propose a learning from demonstration approach that allows the user to simply demonstrate the desired style by driving the car manually. We model the individual style in terms of a cost function and use feature-based inverse reinforcement learning to find the model parameters that fit the observed style best. Once the model has been learned, it can be used to efficiently compute trajectories for the vehicle in autonomous mode. We show that our approach is capable of learning cost functions and reproducing different driving styles using data from real drivers.},
  issn      = {1050-4729},
  journal   = {2015 IEEE International Conference on Robotics and Automation (ICRA)},
  keywords  = {learning systems, mobile robots, acceleration profiles, autonomous vehicles, cost function, demonstration approach, feature-based inverse reinforcement learning, learning driving styles, Acceleration, Cost function, Mobile robots, Navigation, Road transportation, Trajectory, Vehicles},
}

@InProceedings{Mainprice2015,
  author    = {Mainprice, Jim, and Hayne, Rafi, and Berenson, Dmitry},
  title     = {Predicting human reaching motion in collaborative tasks using Inverse Optimal Control and iterative re-planning},
  booktitle = {IEEE International Conference on Robotics and Automation (ICRA)},
  year      = {2015},
  pages     = {885--892},
  abstract  = {To enable safe and efficient human-robot collaboration in shared workspaces, it is important for the robot to predict how a human will move when performing a task. While predicting human motion for tasks not known a priori is very challenging, we argue that single-arm reaching motions for known tasks in collaborative settings (which are especially relevant for manufacturing) are indeed predictable. Two hypotheses underlie our approach for predicting such motions: First, that the trajectory the human performs is optimal with respect to an unknown cost function, and second, that human adaptation to their partner's motion can be captured well through iterative replanning with the above cost function. The key to our approach is thus to learn a cost function which &#x201C;explains&#x201D; the motion of the human. To do this, we gather example trajectories from two participants performing a collaborative assembly task using motion capture. We then use Inverse Optimal Control to learn a cost function from these trajectories. Finally, we predict a human's motion for a given task by iteratively replanning a trajectory for a 23 DoF human kinematic model using the STOMP algorithm with the learned cost function in the presence of a moving collaborator. Our results suggest that our method outperforms baseline methods and generalizes well for tasks similar to those that were demonstrated.},
  issn      = {1050-4729},
  journal   = {2015 IEEE International Conference on Robotics and Automation (ICRA)},
  keywords  = {human-robot interaction, iterative methods, optimal control, path planning, STOMP algorithm, collaborative tasks, cost function, human kinematic model, human reaching motion prediction, human-robot collaboration, inverse optimal control, iterative re-planning, motion capture, stochastic trajectory optimization for motion planning, Collaboration, Cost function, Hidden Markov models, Optimal control, Planning, Prediction algorithms, Trajectory},
}

@Article{Mainprice2016,
  author   = {Mainprice, Jim, and Hayne, Rafi, and Berenson, Dmitry},
  title    = {Goal Set Inverse Optimal Control and Iterative Replanning for Predicting Human Reaching Motions in Shared Workspaces},
  journal  = {IEEE Transactions on Robotics},
  year     = {2016},
  volume   = {32},
  number   = {4},
  pages    = {897-908},
  month    = {Aug},
  issn     = {1552-3098},
  abstract = {To enable safe and efficient human-robot collaboration in shared workspaces, it is important for the robot to predict how a human will move when performing a task. While predicting human motion for tasks not known a priori is very challenging, we argue that single-arm reaching motions for known tasks in collaborative settings (which are especially relevant for manufacturing) are indeed predictable. Two hypotheses underlie our approach for predicting such motions: First, that the trajectory the human performs is optimal with respect to an unknown cost function, and second, that human adaptation to their partner's motion can be captured well through iterative replanning with the above cost function. The key to our approach is thus to learn a cost function that “explains” the motion of the human. To do this, we gather example trajectories from pairs of participants performing a collaborative assembly task using motion capture. We then use inverse optimal control to learn a cost function from these trajectories. Finally, we predict reaching motions from the human's current configuration to a task-space goal region by iteratively replanning a trajectory using the learned cost function. Our planning algorithm is based on the trajectory optimizer: stochastic trajectory optimizer for motion planning [1]; it plans for a 23-degree-of-freedom human kinematic model and accounts for the presence of a moving collaborator and obstacles in the environment. Our results suggest that in most cases, our method outperforms baseline methods when predicting motions. We also show that our method outperforms baselines for predicting human motion when a human and a robot share the workspace.},
  doi      = {10.1109/TRO.2016.2581216},
  keywords = {human-robot interaction;learning systems;optimal control;path planning;stochastic systems;trajectory control;23-degree-of-freedom human kinematic model;collaborative assembly task;cost function learning;goal set inverse optimal control;human reaching motion prediction;human-robot collaboration;iterative replanning;motion capture;motion planning;single-arm reaching motions;stochastic trajectory optimizer;Collaboration;Cost function;Hidden Markov models;Optimal control;Planning;Robots;Trajectory;Human-robot interaction, machine learning, motion analysis, motion planning, robot motion},
}

@Article{Freeman1996,
  author  = {Freeman, R. and Kokotovic, P.},
  journal = {SIAM Journal on Control and Optimization},
  title   = {Inverse Optimality in Robust Stabilization},
  year    = {1996},
  number  = {4},
  pages   = {1365-1391},
  volume  = {34},
  doi     = {10.1137/S0363012993258732},
  eprint  = {https://doi.org/10.1137/S0363012993258732},
  url     = {https://doi.org/10.1137/S0363012993258732},
}

@Article{Krstic1998,
  author   = {M. Krstic and Zhong-Hua Li},
  title    = {Inverse optimal design of input-to-state stabilizing nonlinear controllers},
  journal  = {IEEE Transactions on Automatic Control},
  year     = {1998},
  volume   = {43},
  number   = {3},
  pages    = {336-350},
  month    = {Mar},
  issn     = {0018-9286},
  abstract = {We show that input-to-state stabilizability (as defined by Sontag,1989, 1995) is both necessary and sufficient for the solvability of a Hamilton-Jacobi-Isaacs equation associated with a meaningful differential game problem similar to, but more general than, the “nonlinear H∞” problem. The significance of the result stems from the fact that constructive solutions to the input-to-state stabilization problem are available (presented in the paper) and that, as shown here, inverse optimal controllers possess margins on input-to-state stability against a certain class of input unmodeled dynamics. Rather than completion of squares, the main tools in our analysis are Legendre-Fenchel transformations and the general form of Young's inequality},
  doi      = {10.1109/9.661589},
  keywords = {Jacobian matrices;control system synthesis;differential games;inverse problems;nonlinear control systems;optimal control;stability;Hamilton-Jacobi-Isaacs equation solvability;Legendre-Fenchel transformations;Young inequality;differential game problem;input-to-state stabilizability;input-to-state stabilizing nonlinear controllers;inverse optimal controllers;inverse optimal design;necessary and sufficient condition;nonlinear H∞ problem;Backstepping;Control theory;Differential equations;Kalman filters;Lyapunov method;Nonlinear equations;Optimal control;Partial differential equations;Robust control;Stability},
}

@Article{Faruque2018,
  author   = {Faruque, Imraan A. and Muijres, Florian T. and Macfarlane, Kenneth M. and Kehlenbeck, Andrew and Humbert, J. Sean},
  title    = {Identification of optimal feedback control rules from micro-quadrotor and insect flight trajectories},
  journal  = {Biological Cybernetics},
  year     = {2018},
  volume   = {112},
  number   = {3},
  pages    = {165--179},
  month    = {Jun},
  issn     = {1432-0770},
  abstract = {This paper presents ``optimal identification,'' a framework for using experimental data to identify the optimality conditions associated with the feedback control law implemented in the measurements. The technique compares closed loop trajectory measurements against a reduced order model of the open loop dynamics, and uses linear matrix inequalities to solve an inverse optimal control problem as a convex optimization that estimates the controller optimality conditions. In this study, the optimal identification technique is applied to two examples, that of a millimeter-scale micro-quadrotor with an engineered controller on board, and the example of a population of freely flying Drosophila hydei maneuvering about forward flight. The micro-quadrotor results show that the performance indices used to design an optimal flight control law for a micro-quadrotor may be recovered from the closed loop simulated flight trajectories, and the Drosophila results indicate that the combined effect of the insect longitudinal flight control sensing and feedback acts principally to regulate pitch rate.},
  day      = {01},
  doi      = {10.1007/s00422-017-0742-x},
  url      = {https://doi.org/10.1007/s00422-017-0742-x},
}

@Article{Berret2008,
  author    = {Berret, Bastien AND Darlot, Christian AND Jean, Frédéric AND Pozzo, Thierry AND Papaxanthis, Charalambos AND Gauthier, Jean Paul},
  title     = {The Inactivation Principle: Mathematical Solutions Minimizing the Absolute Work and Biological Implications for the Planning of Arm Movements},
  journal   = {PLOS Computational Biology},
  year      = {2008},
  volume    = {4},
  number    = {10},
  pages     = {1-25},
  month     = {10},
  abstract  = {Author Summary When performing reaching and grasping movements, the brain has to choose one trajectory among an infinite set of possibilities. Nevertheless, because human and animal movements provide highly stereotyped features, motor strategies used by the brain were assumed to be optimal according to certain optimality criteria. In this study, we propose a theoretical model for motor planning of arm movements that minimizes a compromise between the absolute work exerted by the muscles and the integral of the squared acceleration. We demonstrate that under these assumptions agonistic and antagonistic muscles are inactivated during overlapping periods of time for quick enough movements. Moreover, it is shown that only this type of criterion can predict these inactivation periods. Finally, experimental evidence is in agreement with the predictions of the model. Indeed, we report the existence of simultaneous inactivation of opposing muscles during fast vertical arm movements. Therefore, this study suggests that biological movements partly optimize the energy expenditure, integrating both inertial and gravitational forces during the motor planning process.},
  doi       = {10.1371/journal.pcbi.1000194},
  publisher = {Public Library of Science},
  url       = {https://doi.org/10.1371/journal.pcbi.1000194},
}

@Article{Chitour2012,
  author  = {Chitour, Y. and Jean, F. and Mason, P.},
  journal = {SIAM Journal on Control and Optimization},
  title   = {Optimal Control Models of Goal-oriented Human Locomotion},
  year    = {2012},
  number  = {1},
  pages   = {147-170},
  volume  = {50},
  doi     = {10.1137/100799344},
  eprint  = {https://doi.org/10.1137/100799344},
  url     = {https://doi.org/10.1137/100799344},
}

@Article{Chittaro2013,
  author   = {Chittaro, F. C. and Jean, F. and Mason, P.},
  title    = {On Inverse Optimal Control Problems of Human Locomotion: Stability and Robustness of the Minimizers},
  journal  = {Journal of Mathematical Sciences},
  year     = {2013},
  volume   = {195},
  number   = {3},
  pages    = {269--287},
  month    = {Dec},
  issn     = {1573-8795},
  abstract = {In recent papers, models of human locomotion by means of optimal control problems have been proposed. In this paradigm, the trajectories are assumed to be solutions of an optimal control problem whose cost has to be determined. The purpose of the present paper is to analyze the class of optimal control problems defined in this way. We prove strong convergence results for their solutions, on the one hand, for perturbations of the initial and final points (stability), and, on the other hand, for perturbations of the cost (robustness).},
  day      = {01},
  doi      = {10.1007/s10958-013-1579-z},
  url      = {https://doi.org/10.1007/s10958-013-1579-z},
}

@Article{Berret2011,
  author    = {Berret, Bastien AND Chiovetto, Enrico AND Nori, Francesco AND Pozzo, Thierry},
  title     = {Evidence for Composite Cost Functions in Arm Movement Planning: An Inverse Optimal Control Approach},
  journal   = {PLOS Computational Biology},
  year      = {2011},
  volume    = {7},
  number    = {10},
  pages     = {1-18},
  month     = {10},
  abstract  = {Author Summary To reach an object, the brain has to select among a set of possible arm trajectories that displace the hand from an initial to a final desired position. Because of the intrinsic redundancy characterizing the human arm, the number of admissible joint trajectories toward the goal is generally infinite. However, many studies have demonstrated that the range of actual trajectories can be limited to those that result from the fulfillment of some optimal rules. Various cost functions were shown to be relevant in the literature. A peculiar aspect of most of these costs is that each one of them aims at optimizing one specific feature of the movement. The necessary motor flexibility of everyday life, however, might rely on the combination of such cost functions rather than on a single one. Testing this cost combination hypothesis has never been attempted. To this aim we propose a reaching task involving target redundancy to facilitate the comparisons of different candidate costs and to identify the best-fitting one (possibly composite). Using a numerical inverse optimal control method, we show that most participants produced movements corresponding to a strict combination of two subjective costs linked to the mechanical energy consumption and the joint-level smoothness.},
  doi       = {10.1371/journal.pcbi.1002183},
  publisher = {Public Library of Science},
  url       = {https://doi.org/10.1371/journal.pcbi.1002183},
}

@Article{Park1975,
  author   = {J. G. Park and K. Y. Lee},
  title    = {An Inverse Optimal Control Problem and Its Application to the Choice of Performance Index for Economic Stabilization Policy},
  journal  = {IEEE Transactions on Systems, Man, and Cybernetics},
  year     = {1975},
  volume   = {SMC-5},
  number   = {1},
  pages    = {64-76},
  month    = {Jan},
  issn     = {0018-9472},
  abstract = {The specification of a performance criterion is one of the basic requirements for the formal analysis of quantitative decision processes. A procedure of quantitatively selecting the performance index for economic stabilization policy by solving the so-called inverse optimal control problem is developed. When a closed-loop system with a known control policy is given, the inverse optimal control problem is to determine performance indices for which the given control rule is optimal. A sufficient condition is developed for the solution of the inverse problem for long-run economic stabilization policy, and an explicit solution is obtained for short-run economic stabilization policy by considering a special case where the performance index does not penalize the costs of implementing control policies. The solution of the inverse problem is found to be not unique in general, which implies that the optimal control policies are fairly robust against different performance indices. Also, it is found that the solution of the inverse problem for a linear regulator holds true for the linear tracking problem, which makes the analysis much simpler. A procedure is developed for the selection of the performance index along with the optimal feedback control policy by which the economic system is to reveal the desired characteristics. The procedure demonstrates the determination of the steady states as policy goals, the computation of the feedback control policy, and the construction of a performance index, through a small econometric model.},
  doi      = {10.1109/TSMC.1975.5409156},
  keywords = {Control systems;Costs;Econometrics;Feedback control;Inverse problems;Optimal control;Performance analysis;Regulators;Robust control;Sufficient conditions},
}

@Article{Sugimoto1988,
  author    = {Kenji Sugimoto and Yutaka Yamamoto},
  journal   = {International Journal of Control},
  title     = {Solution to the inverse regulator problem for discrete-time systems},
  year      = {1988},
  number    = {3},
  pages     = {1285-1300},
  volume    = {48},
  abstract  = {A complete solution is given for the inverse problem of LQ optimal regulators for the discrete-time multi-input case. The Kalman equation for discrete-time systems is derived to characterize the optimal regulators. It is then shown that this equation holds for some quadratic weighting if and only if the feedback satisfies a condition corresponding to the circle criterion for continuous-time systems. The optimality criterion given here consists of this condition and an additional condition to ensure detectability. An example is given to illustrate the results.},
  doi       = {10.1080/00207178808906246},
  eprint    = {https://doi.org/10.1080/00207178808906246},
  publisher = {Taylor \& Francis},
  url       = {https://doi.org/10.1080/00207178808906246},
}

@Article{Thau1967,
  author   = {F. Thau},
  title    = {On the inverse optimum control problem for a class of nonlinear autonomous systems},
  journal  = {IEEE Transactions on Automatic Control},
  year     = {1967},
  volume   = {12},
  number   = {6},
  pages    = {674-681},
  month    = {December},
  issn     = {0018-9286},
  abstract = {Some aspects of the inverse optimum control problem are considered for a class of nonlinear autonomous systems. A closed-loop system with a known control law is given; the problem is to determine performance criteria for which the given control law is optimum. Algebraic conditions that must be satisfied by a class of scalar performance criteria of the formV=intmin{t}max{infty}[q(x)+h(u)]d_{tau}are obtained. It is shown that if the value of the optimum V0is required to be a quadratic formV^{o} = frac{1}{2}x'Mxof the current statex, and if certain state variables cannot be measured, thenMcannot be positive definite. The inverse optimum control problem corresponding to the problem of Lur'e is considered. Examples are given to illustrate the techniques and to compare the properties of a linear and nonlinear system having the same optimum performanceV^{0}(x).},
  doi      = {10.1109/TAC.1967.1098741},
  keywords = {Inverse optimal control problem;Nonlinear systems;Optimal control;Aerodynamics;Control systems;Control theory;Current measurement;Inverse problems;Kalman filters;Linear systems;Nonlinear control systems;Nonlinear systems;Optimal control},
}

@InProceedings{Ng2000,
  author    = {Andrew Y. Ng and Stuart Russell},
  title     = {Algorithms for Inverse Reinforcement Learning},
  booktitle = {in Proc. 17th International Conf. on Machine Learning},
  year      = {2000},
  pages     = {663--670},
  publisher = {Morgan Kaufmann},
}

@Article{Kong2012,
  author    = {He Kong and Graham Goodwin and Maria Seron},
  journal   = {International Journal of Control},
  title     = {A revisit to inverse optimality of linear systems},
  year      = {2012},
  number    = {10},
  pages     = {1506-1514},
  volume    = {85},
  abstract  = {In this article, we revisit the problem of inverse optimality for linear systems. By applying certain explicit formulae for coprime matrix fraction descriptions (CMFD) of linear systems, we propose a necessary and sufficient condition for a given stable state feedback law to be optimal for some quadratic performance index. Compared to existing results in the literature, the proposed condition is simpler to check and interpret. Moreover, it reduces the redundancy in the solutions of the associated algebraic Riccati equation (ARE). As a direct application of the proposed results, we consider the problem of inverse optimality of observer-based state feedback. To be specific, for the case where the state is not fully known, we consider the inverse optimality problem of an observer-based state feedback for the closed-loop system augmented by an observer. More precisely, it is shown that the observer-based state feedback is inverse optimal for the closed-loop system with some general forms of cost functions, only if the original state feedback is inverse optimal for the original system with certain cost functions, irrespective of the choice of the observer. This coincides with existing results in the literature. Some other applications of the proposed results are also discussed. We also illustrate the proposed results through an example.},
  doi       = {10.1080/00207179.2012.691180},
  eprint    = {https://doi.org/10.1080/00207179.2012.691180},
  publisher = {Taylor \& Francis},
  url       = {https://doi.org/10.1080/00207179.2012.691180},
}

@Article{Moylan1973,
  author    = {Moylan, Peter and Anderson, D.O. Brian},
  title     = {Nonlinear regulator and an inverse optimal control problem},
  journal   = {IEEE Transactions on Automatic Control},
  year      = {1973},
  volume    = {18},
  pages     = {460- 465},
  month     = {11},
  booktitle = {Automatic Control, IEEE Transactions on},
}

@Article{Casti1980,
  author   = {Casti, J.},
  title    = {On the general inverse problem of optimal control theory},
  journal  = {Journal of Optimization Theory and Applications},
  year     = {1980},
  volume   = {32},
  number   = {4},
  pages    = {491--497},
  month    = {Dec},
  issn     = {1573-2878},
  abstract = {The general inverse problem of optimal control is considered from a dynamic programming point of view. Necessary and sufficient conditions are developed which two integral criteria must satisfy if they are to yield the same optimal feedback law, the dynamics being fixed. Specializing to the linear-quadratic case, it is shown how the general results given here recapture previously obtained results for quadratic criteria with linear dynamics.},
  day      = {01},
  doi      = {10.1007/BF00934036},
  url      = {https://doi.org/10.1007/BF00934036},
}

@Article{Sugimoto1989,
  author    = {Sugimoto, Kenji and Yamamoto, Yutaka},
  title     = {On successive pole assignment by linear-quadratic optimal feedbacks},
  journal   = {Linear Algebra and its Applications},
  year      = {1989},
  volume    = {122},
  pages     = {697--723},
  publisher = {North-Holland},
}

@Article{Mombaur2010,
  author   = {Mombaur, Katja and Truong, Anh and Laumond, Jean-Paul},
  title    = {From human to humanoid locomotion---an inverse optimal control approach},
  journal  = {Autonomous Robots},
  year     = {2010},
  volume   = {28},
  number   = {3},
  pages    = {369--383},
  month    = {Apr},
  issn     = {1573-7527},
  abstract = {The purpose of this paper is to present inverse optimal control as a promising approach to transfer biological motions to robots. Inverse optimal control helps (a) to understand and identify the underlying optimality criteria of biological motions based on measurements, and (b) to establish optimal control models that can be used to control robot motion. The aim of inverse optimal control problems is to determine---for a given dynamic process and an observed solution---the optimization criterion that has produced the solution. Inverse optimal control problems are difficult from a mathematical point of view, since they require to solve a parameter identification problem inside an optimal control problem. We propose a pragmatic new bilevel approach to solve inverse optimal control problems which rests on two pillars: an efficient direct multiple shooting technique to handle optimal control problems, and a state-of-the art derivative free trust region optimization technique to guarantee a match between optimal control problem solution and measurements. In this paper, we apply inverse optimal control to establish a model of human overall locomotion path generation to given target positions and orientations, based on newly collected motion capture data. It is shown how the optimal control model can be implemented on the humanoid robot HRP-2 and thus enable it to autonomously generate natural locomotion paths.},
  day      = {01},
  doi      = {10.1007/s10514-009-9170-7},
  url      = {https://doi.org/10.1007/s10514-009-9170-7},
}

@InProceedings{Puydupin-Jamin2012,
  author    = {A. S. Puydupin-Jamin and M. Johnson and T. Bretl},
  title     = {A convex approach to inverse optimal control and its application to modeling human locomotion},
  booktitle = {IEEE International Conference on Robotics and Automation},
  year      = {2012},
  pages     = {531-536},
  month     = {May},
  abstract  = {Inverse optimal control is the problem of computing a cost function that would have resulted in an observed sequence of decisions. The standard formulation of this problem assumes that decisions are optimal and tries to minimize the difference between what was observed and what would have been observed given a candidate cost function. We assume instead that decisions are only approximately optimal and try to minimize the extent to which observed decisions violate first-order necessary conditions for optimality. For a discrete-time optimal control system with a cost function that is a linear combination of known basis functions, this formulation leads to an efficient method of solution as an unconstrained least-squares problem. We apply this approach to both simulated and experimental data to obtain a simple model of human walking trajectories. This model might subsequently be used either for control of a humanoid robot or for predicting human motion when moving a robot through crowded areas.},
  doi       = {10.1109/ICRA.2012.6225317},
  issn      = {1050-4729},
  keywords  = {biocontrol;biomechanics;discrete time systems;humanoid robots;least squares approximations;optimal control;trajectory control;convex approach;cost function computation problem;difference minimization;discrete-time optimal control system;first-order necessary conditions;human locomotion modeling;human motion prediction;human walking trajectories;humanoid robot;inverse optimal control;unconstrained least-squares problem;Cost function;Data models;Humans;Mathematical model;Optimal control;Trajectory},
}

@InProceedings{Ratliff2006,
  author    = {Ratliff, Nathan D. and Bagnell, J. Andrew and Zinkevich, Martin A.},
  title     = {Maximum Margin Planning},
  booktitle = {Proceedings of the 23rd International Conference on Machine Learning},
  year      = {2006},
  series    = {ICML '06},
  pages     = {729--736},
  address   = {New York, NY, USA},
  publisher = {ACM},
  acmid     = {1143936},
  doi       = {10.1145/1143844.1143936},
  isbn      = {1-59593-383-2},
  location  = {Pittsburgh, Pennsylvania, USA},
  numpages  = {8},
  url       = {http://doi.acm.org/10.1145/1143844.1143936},
}

@Article{Zelenko2006,
  author   = {Zelenko, I.},
  title    = {On geodesic equivalence of Riemannian metrics and sub-Riemannian metrics on distributions of corank 1},
  journal  = {Journal of Mathematical Sciences},
  year     = {2006},
  volume   = {135},
  number   = {4},
  pages    = {3168--3194},
  month    = {Jun},
  issn     = {1573-8795},
  note     = {{Sovrem. Mat. Prilozh.} No.\ 21, {Geom. Zadachi Teor. Upr.}, 79--105, 2004},
  abstract = {The present paper is devoted to the problem of (local) geodesic equivalence of Riemannian metrics and sub-Riemannian metrics on generic corank 1 distributions. Using the Pontryagin maximum principle, we treat Riemannian and sub-Riemannian cases in a unified way and obtain some algebraic necessary conditions for the geodesic equivalence of (sub-)Riemannian metrics. In this way, first we obtain a new elementary proof of the classical Levi-Civita theorem on the classification of all Riemannian geodesically equivalent metrics in a neighborhood of the so-called regular (stable) point w.r.t. these metrics. Second, we prove that sub-Riemannian metrics on contact distributions are geodesically equivalent iff they are constantly proportional. Then we describe all geodesically equivalent sub-Riemannian metrics on quasi-contact distributions. Finally, we give a classification of all pairs of geodesically equivalent Riemannian metrics on a surface that are proportional at an isolated point. This is the simplest case, which was not covered by Levi-Civita's theorem.},
  day      = {01},
  doi      = {10.1007/s10958-006-0151-5},
  url      = {https://doi.org/10.1007/s10958-006-0151-5},
}

@Article{Matveev-Topalov2003,
  author   = {Topalov, Peter and Matveev, Vladimir S.},
  title    = {Geodesic Equivalence via Integrability},
  journal  = {Geometriae Dedicata},
  year     = {2003},
  volume   = {96},
  number   = {1},
  pages    = {91--115},
  month    = {Feb},
  issn     = {1572-9168},
  abstract = {We suggest a construction that, given an orbital diffeomorphism between two Hamiltonian systems, produces integrals of them. We treat geodesic equivalence of metrics as the main example of it. In this case, the integrals commute; they are functionally independent if the eigenvalues of the tensor gi$\alpha$g{\textasciimacron}$\alpha$j are all different; if the eigenvalues are all different at least at one point then they are all different at almost each point and the geodesic flows of the metrics are Liouville integrable. This gives us topological obstacles to geodesic equivalence.},
  day      = {01},
  doi      = {10.1023/A:1022166218282},
  url      = {https://doi.org/10.1023/A:1022166218282},
}

@Article{Levi-Civita1896,
  author    = {Levi-Civita, Tullio},
  title     = {Sulle trasformazioni delle equazioni dinamiche},
  journal   = {Annali di Matematica Pura ed Applicata (1867-1897)},
  year      = {1896},
  volume    = {24},
  number    = {1},
  pages     = {255--300},
  publisher = {Springer},
}

@Article{Beltrami1869,
  author    = {Beltrami, Eugenio},
  title     = {Teoria fondamentale degli spazii di curvatura costante},
  journal   = {Annali di Matematica Pura ed Applicata},
  year      = {1868},
  volume    = {2},
  number    = {1},
  pages     = {232--255},
  publisher = {Springer},
}

@Article{Gauthier2010,
  author   = {Gauthier, Jean-Paul and Berret, Bastien and Jean, Fr{\'e}d{\'e}ric},
  title    = {A biomechanical inactivation principle},
  journal  = {Proceedings of the Steklov Institute of Mathematics},
  year     = {2010},
  volume   = {268},
  number   = {1},
  pages    = {93--116},
  month    = {Apr},
  issn     = {1531-8605},
  abstract = {This paper develops the mathematical side of a theory of inactivations in human biomechanics. This theory has been validated by practical experiments, including zero-gravity experiments. The theory mostly relies on Pontryagin's maximum principle on the one side and on transversality theory on the other side. It turns out that the periods of silence in the activation of muscles that are observed in practice during the motions of the arm can appear only if ``something like the energy expenditure'' is minimized. Conversely, minimization of a criterion taking into account the ``energy expenditure'' guaranties the presence of these periods of silence, for sufficiently short movements.},
  day      = {01},
  doi      = {10.1134/S0081543810010098},
  url      = {https://doi.org/10.1134/S0081543810010098},
}

@Article{Agrachev2017,
  author  = {A. Agrachev, and D. Barilari, and U. Boscain},
  title   = {Introduction to Riemannian and sub-Riemannian geometry},
  journal = {Lecture notes available at http://webusers.imj-prg.fr/$\sim$davide.barilari/Notes.php, preprint SISSA 09/2012/M. Version Nov 17, 2017.},
  year    = {2017},
}

@Article{AgrachevBarilariRizzi,
  author  = {Agrachev, Andrei and Barilari, Davide and Rizzi, Luca},
  journal = {Memoirs of the AMS},
  title   = {Curvature: a variational approach},
  year    = {2018},
  number  = {1225},
  volume  = {256},
  doi     = {10.1090/memo/1225},
}

@Article{Agrachev1997,
  author   = {Agrachev, A. A. and Gamkrelidze, R. V.},
  title    = {Feedback-invariant optimal control theory and differential geometry---I. Regular extremals},
  journal  = {Journal of Dynamical and Control Systems},
  year     = {1997},
  volume   = {3},
  number   = {3},
  pages    = {343--389},
  month    = {Jul},
  issn     = {1573-8698},
  abstract = {A feedback-invariant approach to smooth optimal control problems is considered. A Hamiltonian method of investigating regular extremals is developed, analogous to the differential-geometric method of investigating Riemannian geodesics in terms of the Levi-Civita connection and the curvature tensor.},
  day      = {01},
  doi      = {10.1007/BF02463256},
  url      = {https://doi.org/10.1007/BF02463256},
}

@Article{Agrachev2015,
  author   = {Agrachev, Andrei and Rizzi, Luca and Silveira, Pavel},
  title    = {On Conjugate Times of LQ Optimal Control Problems},
  journal  = {Journal of Dynamical and Control Systems},
  year     = {2015},
  volume   = {21},
  number   = {4},
  pages    = {625--641},
  month    = {Oct},
  issn     = {1573-8698},
  abstract = {Motivated by the study of linear quadratic optimal control problems, we consider a dynamical system with a constant, quadratic Hamiltonian, and we characterize the number of conjugate times in terms of the spectrum of the Hamiltonian vector field                                                                                                                                                                       H                                                {\textrightarrow}                                                                              {\$}{\backslash}vec {\{}H{\}}{\$}                . We prove the following dichotomy: the number of conjugate times is identically zero or grows to infinity. The latter case occurs if and only if                                                                                                                                                                       H                                                {\textrightarrow}                                                                              {\$}{\backslash}vec {\{}H{\}}{\$}                 has at least one Jordan block of odd dimension corresponding to a purely imaginary eigenvalue. As a byproduct, we obtain bounds from below on the number of conjugate times contained in an interval in terms of the spectrum of                                                                                                                                                                       H                                                {\textrightarrow}                                                                              {\$}{\backslash}vec {\{}H{\}}{\$}                .},
  day      = {01},
  doi      = {10.1007/s10883-014-9251-6},
  url      = {https://doi.org/10.1007/s10883-014-9251-6},
}

@Article{Agrachev2002,
  author   = {Agrachev, A. A. and Zelenko, I.},
  title    = {Geometry of Jacobi Curves. I},
  journal  = {Journal of Dynamical and Control Systems},
  year     = {2002},
  volume   = {8},
  number   = {1},
  pages    = {93--140},
  month    = {Jan},
  issn     = {1573-8698},
  abstract = {Jacobi curves are deep generalizations of the spaces of ``Jacobi fields'' along Riemannian geodesics. Actually, Jacobi curves are curves in the Lagrange Grassmannians. In our paper we develop differential geometry of these curves which provides basic feedback or gauge invariants for a wide class of smooth control systems and geometric structures. Two principal invariants are the generalized Ricci curvature, which is an invariant of the parametrized curve in the Lagrange Grassmannian endowing the curve with a natural projective structure, and a fundamental form, which is a fourth-order differential on the curve. The so-called rank 1 curves are studied in more detail. Jacobi curves of this class are associated with systems with scalar controls and with rank 2 vector distributions.},
  day      = {01},
  doi      = {10.1023/A:1013904801414},
  url      = {https://doi.org/10.1023/A:1013904801414},
}

@Article{Barilari2018,
  author  = {Barilari, D. and Boarotto, F.},
  journal = {SIAM Journal on Control and Optimization},
  title   = {On the Set of Points of Smoothness for the Value Function of Affine Optimal Control Problems},
  year    = {2018},
  number  = {2},
  pages   = {649-671},
  volume  = {56},
  doi     = {10.1137/17M1123948},
  eprint  = {https://doi.org/10.1137/17M1123948},
  url     = {https://doi.org/10.1137/17M1123948},
}

@InBook{Bellaieche1996,
  pages     = {1--78},
  title     = {The tangent space in sub-Riemannian geometry},
  publisher = {Birkh{\"a}user Basel},
  year      = {1996},
  author    = {Bella{\"i}che, Andr{\'e}},
  editor    = {Bella{\"i}che, Andr{\'e} and Risler, Jean-Jacques},
  address   = {Basel},
  isbn      = {978-3-0348-9210-0},
  abstract  = {Tangent spaces of a sub-Riemannian manifold are themselves sub-Riemannian manifolds. They can be defined as metric spaces, using Gromov's definition of tangent spaces to a metric space, and they turn out to be sub-Riemannian manifolds. Moreover, they come with an algebraic structure: nilpotent Lie groups with dilations. In the classical, Riemannian, case, they are indeed vector spaces, that is, abelian groups with dilations. Actually, the above is true only for regular points. At singular points, instead of nilpotent Lie groups one gets quotient spaces G/H of such groups G.},
  booktitle = {Sub-Riemannian Geometry},
  doi       = {10.1007/978-3-0348-9210-0_1},
  url       = {https://doi.org/10.1007/978-3-0348-9210-0_1},
}

@Article{Benenti1997,
  author  = {Benenti, Sergio},
  journal = {Journal of Mathematical Physics},
  title   = {Intrinsic characterization of the variable separation in the Hamilton-Jacobi equation},
  year    = {1997},
  number  = {12},
  pages   = {6578-6602},
  volume  = {38},
  doi     = {10.1063/1.532226},
  eprint  = {https://doi.org/10.1063/1.532226},
  url     = {https://doi.org/10.1063/1.532226},
}

@Article{Benenti2016,
  author    = {Benenti, Sergio},
  title     = {Separability in Riemannian manifolds},
  journal   = {SIGMA. Symmetry, Integrability and Geometry: Methods and Applications},
  year      = {2016},
  volume    = {12},
  number    = {13},
  publisher = {SIGMA. Symmetry, Integrability and Geometry: Methods and Applications},
}

@Article{Berret2016,
  author    = {Berret, Bastien and Jean, Fr{\'e}d{\'e}ric},
  title     = {Why Don{\textquoteright}t We Move Slower? The Value of Time in the Neural Control of Action},
  journal   = {Journal of Neuroscience},
  year      = {2016},
  volume    = {36},
  number    = {4},
  pages     = {1056--1070},
  issn      = {0270-6474},
  abstract  = {To want something now rather than later is a common attitude that reflects the brain{\textquoteright}s tendency to value the passage of time. Because the time taken to accomplish an action inevitably delays task achievement and reward acquisition, this idea was ported to neural movement control within the {\textquotedblleft}cost of time{\textquotedblright} theory. This theory provides a normative framework to account for the underpinnings of movement time formation within the brain and the origin of a self-selected pace in human and animal motion. Then, how does the brain exactly value time in the control of action? To tackle this issue, we used an inverse optimal control approach and developed a general methodology allowing to squarely sample infinitesimal values of the time cost from experimental motion data. The cost of time underlying saccades was found to have a concave growth, thereby confirming previous results on hyperbolic reward discounting, yet without making any prior assumption about this hypothetical nature. For self-paced reaching, however, movement time was primarily valued according to a striking sigmoidal shape; its rate of change consistently presented a steep rise before a maximum was reached and a slower decay was observed. Theoretical properties of uniqueness and robustness of the inferred time cost were established for the class of problems under investigation, thus reinforcing the significance of the present findings. These results may offer a unique opportunity to uncover how the brain values the passage of time in healthy and pathological motor control and shed new light on the processes underlying action invigoration.SIGNIFICANCE STATEMENT Movement time is a fundamental characteristic of neural motor control, but the principles underlying its formation remain little known. This work addresses that question within the inverse optimal control framework where the challenge is to uncover what optimality criterion underlies a system{\textquoteright}s behavior. Here we rely on the {\textquotedblleft}cost of time{\textquotedblright} theory that finds its roots into the brain{\textquoteright}s tendency to discount the actual value of future reward. It asserts that the time elapsed until action completion entails a cost, thereby making slow moves nonoptimal. By means of a thorough theoretical analysis, the present article shows how to sample the infinitesimal values of the time cost without prior assumption about its hypothetical nature and emphasizes its sigmoidal shape for reaching.},
  doi       = {10.1523/JNEUROSCI.1921-15.2016},
  eprint    = {http://www.jneurosci.org/content/36/4/1056.full.pdf},
  publisher = {Society for Neuroscience},
  url       = {http://www.jneurosci.org/content/36/4/1056},
}

@Article{Bonnard2007,
  author    = {Bonnard, Bernard and Caillau, Jean-Baptiste and Tr\'{e}lat, Emmanuel},
  title     = {Second order optimality conditions in the smooth case and applications in optimal control},
  journal   = {ESAIM: Control, Optimisation and Calculus of Variations},
  year      = {2007},
  volume    = {13},
  number    = {2},
  pages     = {207-236},
  issn      = {1292-8119},
  abstract  = {The aim of this article is to present algorithms to compute the first conjugate time along a smooth extremal curve, where the trajectory ceases to be optimal. It is based on recent theoretical developments of geometric optimal control, and the article contains a review of second order optimality conditions. The computations are related to a test of positivity of the intrinsic second order derivative or a test of singularity of the extremal flow. We derive an algorithm called COTCOT (Conditions of Order Two and COnjugate Times), available on the web, and apply it to the minimal time problem of orbit transfer, and to the attitude control problem of a rigid spacecraft. This algorithm involves both normal and abnormal cases.},
  database  = {Cambridge Core},
  doi       = {10.1051/cocv:2007012},
  edition   = {2007/05/12},
  keywords  = {Conjugate point, second-order intrinsic derivative, Lagrangian singularity, Jacobi field, orbit transfer, attitude control},
  publisher = {EDP Sciences},
  url       = {https://www.cambridge.org/core/article/second-order-optimality-conditions-in-the-smooth-case-and-applications-in-optimal-control/DB7C6A7E5BDF2623A1DDC009557A0C9E},
}

@Article{deRham1952,
  author    = {De Rham, Georges},
  title     = {Sur la r{\'e}ductibilit{\'e} d'un espace de Riemann},
  journal   = {Commentarii Mathematici Helvetici},
  year      = {1952},
  volume    = {26},
  number    = {1},
  pages     = {328--344},
  publisher = {Springer},
}

@Article{Dini1870,
  author  = {Dini, Ulisse},
  title   = {Sopra un problema che si presenta nella teoria generale delle rappresentazioni geografiche di una superficie su di un'altra},
  journal = {Annali di Matematica Pura ed Applicata (1867-1897)},
  year    = {1869},
  volume  = {3},
  number  = {1},
  pages   = {269--293},
  month   = {Oct},
  issn    = {0373-3114},
  day     = {01},
  doi     = {10.1007/BF02422982},
  url     = {https://doi.org/10.1007/BF02422982},
}

@Article{Eisenhart1923,
  author    = {Luther Pfahler Eisenhart},
  title     = {Symmetric Tensors of the Second Order Whose First Covariant Derivatives are Zero},
  journal   = {Transactions of the American Mathematical Society},
  year      = {1923},
  volume    = {25},
  number    = {2},
  pages     = {297--306},
  issn      = {00029947},
  publisher = {American Mathematical Society},
  url       = {http://www.jstor.org/stable/1989258},
}

@Article{Ferrante2005,
  author   = {Augusto Ferrante and Giovanni Marro and Lorenzo Ntogramatzidis},
  title    = {A parametrization of the solutions of the finite-horizon LQ problem with general cost and boundary conditions},
  journal  = {Automatica},
  year     = {2005},
  volume   = {41},
  number   = {8},
  pages    = {1359 - 1366},
  issn     = {0005-1098},
  abstract = {A generalization of the finite-horizon linear quadratic regulator problem is proposed for LTI continuous-time controllable systems. In particular, a formulation of the linear quadratic (LQ) problem is considered, with affine constraints on the initial and the terminal states and with general quadratic costs in the initial and terminal states. The solution presented is simple and attractive from a computational point of view, and is based on the solutions of an algebraic Riccati equation and of a Lyapunov equation, that enable all the solutions of the Hamiltonian differential equation to be parametrized in closed form.},
  doi      = {https://doi.org/10.1016/j.automatica.2005.01.018},
  keywords = {Finite-horizon LQ problem, Hamiltonian differential equation, Algebraic Riccati equations, Boundary conditions, Optimal cost},
  url      = {http://www.sciencedirect.com/science/article/pii/S0005109805000993},
}

@Article{Gauger1973,
  author    = {Michael A. Gauger},
  title     = {On the Classification of Metabelian Lie Algebras},
  journal   = {Transactions of the American Mathematical Society},
  year      = {1973},
  volume    = {179},
  pages     = {293--329},
  issn      = {00029947},
  abstract  = {The classification of 2-step nilpotent Lie algebras is attacked by a generator-relation method. The main results are in low dimensions or a small number of relations.},
  publisher = {American Mathematical Society},
  url       = {http://www.jstor.org/stable/1996506},
}

@Article{Hamel1903,
  author  = {Hamel, Georg},
  title   = {{\"U}ber die Geometrieen, in denen die Geraden die K{\"u}rzesten sind},
  journal = {Mathematische Annalen},
  year    = {1903},
  volume  = {57},
  number  = {2},
  pages   = {231--264},
  month   = {Jun},
  issn    = {1432-1807},
  day     = {01},
  doi     = {10.1007/BF01444348},
  url     = {https://doi.org/10.1007/BF01444348},
}

@Book{Jean2014,
  title     = {Control of nonholonomic systems: from sub-Riemannian geometry to motion planning},
  publisher = {Springer International Publishing},
  year      = {2014},
  author    = {Jean, Fr{\'e}d{\'e}ric},
}

@Article{Jean2017,
  author   = {Frédéric Jean and Sofya Maslovskaya and Igor Zelenko},
  title    = {Inverse Optimal Control Problem: the Sub-Riemannian Case},
  journal  = {IFAC-PapersOnLine},
  year     = {2017},
  volume   = {50},
  number   = {1},
  pages    = {500 - 505},
  issn     = {2405-8963},
  note     = {20th IFAC World Congress},
  abstract = {The object of this paper is to study the uniqueness of solutions of inverse control problems in the case where the dynamics is given by a control-affine system without drift and the costs are length and energy functionals.},
  doi      = {https://doi.org/10.1016/j.ifacol.2017.08.105},
  keywords = {Optimal control, sub-Riemannian geometry optimal trajectories, geodesics, inverse problem, nonholonomic systems, projective equivalence, affine equivalence},
  url      = {http://www.sciencedirect.com/science/article/pii/S2405896317301398},
}

@Article{Jean2018,
  author  = {Jean, Fr{\'e}d{\'e}ric and Maslovskaya, Sofya and Zelenko, Igor},
  title   = {On projective and affine equivalence of sub-Riemannian metrics},
  journal = {arXiv preprint arXiv:1801.04257},
  year    = {2018},
}

@Article{Kruglikov2015,
  author   = {Boris Kruglikov and Vladimir S Matveev},
  title    = {The geodesic flow of a generic metric does not admit nontrivial integrals polynomial in momenta},
  journal  = {Nonlinearity},
  year     = {2016},
  volume   = {29},
  number   = {6},
  pages    = {1755--1768},
  abstract = {Any smooth geodesic flow is locally Liouville integrable with smooth integrals. We show that generically this fails if we require, in addition, that the integrals are polynomial (or, more generally, analytic) in momenta. Consequently we obtain that a generic real-analytic metric does not admit, even locally, a real-analytic integral.},
  url      = {http://stacks.iop.org/0951-7715/29/i=6/a=1755},
}

@Article{Matveev2003Geodesic,
  author   = {Vladimir S. Matveev},
  title    = {Three-dimensional manifolds having metrics with the same geodesics},
  journal  = {Topology},
  year     = {2003},
  volume   = {42},
  number   = {6},
  pages    = {1371 - 1395},
  issn     = {0040-9383},
  abstract = {We prove that if two Riemannian metrics have the same geodesics on a closed three-dimensional manifold which is homeomorphic neither to a lens space nor to a Seifert manifold with zero Euler number, then the metrics are proportional.},
  doi      = {https://doi.org/10.1016/S0040-9383(03)00004-1},
  keywords = {Geodesic equivalence, Projectively equivalent metrics, Projective connection, Integrable system, Separation of variables, Geodesic rigidity, Liouville metric, Stäckel system, Obstructions to integrability, Local product structure, Lens space},
  url      = {http://www.sciencedirect.com/science/article/pii/S0040938303000041},
}

@Book{Montgomery2002,
  title     = {A tour of subriemannian geometries, their geodesics and applications},
  publisher = {American Mathematical Society},
  year      = {2002},
  author    = {Montgomery, Richard},
  volume    = {92},
  series    = {Mathematical surveys and monographs},
  address   = {Providence, RI},
  url       = {http://cds.cern.ch/record/2122308},
}

@InProceedings{Nori2004,
  author    = {Nori, Francesco and Frezza, Ruggero},
  title     = {Linear optimal control problems and quadratic cost functions estimation},
  booktitle = {12th Mediterranean Conference on Control and Automation},
  year      = {2004},
}

@Article{Priess2015,
  author   = {M. C. Priess and R. Conway and J. Choi and J. M. Popovich and C. Radcliffe},
  title    = {Solutions to the Inverse LQR Problem With Application to Biological Systems Analysis},
  journal  = {IEEE Transactions on Control Systems Technology},
  year     = {2015},
  volume   = {23},
  number   = {2},
  pages    = {770-777},
  month    = {March},
  issn     = {1063-6536},
  abstract = {In this brief, we present a set of techniques for finding a cost function to the time-invariant linear quadratic regulator (LQR) problem in both continuous- and discrete-time cases. Our methodology is based on the solution to the inverse LQR problem, which can be stated as: does a given controller K describe the solution to a time-invariant LQR problem, and if so, what weights Q and R produce K as the optimal solution? Our motivation for investigating this problem is the analysis of motion goals in biological systems. We first describe an efficient linear matrix inequality (LMI) method for determining a solution to the general case of this inverse LQR problem when both the weighting matrices Q and R are unknown. Our first LMI-based formulation provides a unique solution when it is feasible. In addition, we propose a gradient-based, least-squares minimization method that can be applied to approximate a solution in cases when the LMIs are infeasible. This new method is very useful in practice since the estimated gain matrix K from the noisy experimental data could be perturbed by the estimation error, which may result in the infeasibility of the LMIs. We also provide an LMI minimization problem to find a good initial point for the minimization using the proposed gradient descent algorithm. We then provide a set of examples to illustrate how to apply our approaches to several different types of problems. An important result is the application of the technique to human subject posture control when seated on a moving robot. Results show that we can recover a cost function which may provide a useful insight on the human motor control goal.},
  doi      = {10.1109/TCST.2014.2343935},
  keywords = {biology;least squares approximations;linear matrix inequalities;linear quadratic control;minimisation;position control;LMI method;LMI minimization problem;biological systems analysis;cost function;gain matrix;gradient-based least-squares minimization method;human subject posture control;inverse LQR problem;linear matrix inequality;motion goals analysis;moving robot;time-invariant LQR problem;time-invariant linear quadratic regulator;weighting matrix;Biological systems;Cost function;Equations;Inverse problems;Minimization;Motor drives;Noise measurement;Biological system modeling;inverse optimal control problem;system identification},
}

@Article{Tanaka1970,
  author    = {Tanaka, Noboru},
  title     = {On differential systems, graded Lie algebras and pseudo-groups},
  journal   = {Kyoto Journal of Mathematics},
  year      = {1970},
  volume    = {10},
  number    = {1},
  pages     = {1--82},
  doi       = {10.1215/kjm/1250523814},
  fjournal  = {Journal of Mathematics of Kyoto University},
  publisher = {Duke University Press},
  url       = {https://doi.org/10.1215/kjm/1250523814},
}

@Book{Trelat2005,
  title     = {Contr{\^o}le optimal: th{\'e}orie \& applications},
  publisher = {Vuibert Paris},
  year      = {2005},
  author    = {Tr{\'e}lat, Emmanuel},
}

@Article{Weyl1956,
  author  = {Weyl, Hermann},
  title   = {Zur Infinitesimalgeometrie: Einordnung der projektiven und der konformen Auffasung},
  journal = {Nachrichten von der Gesellschaft der Wissenschaften zu G{\"o}ttingen, Mathematisch-Physikalische Klasse},
  year    = {1921},
  volume  = {1921},
  pages   = {99--112},
  note    = {Selecta Hermann Weyl, Birkhauser Verlag, Basel und Stuttgart, 1956.},
}

@Article{Zelenko2007,
  author   = {Igor Zelenko and Chengbo Li},
  title    = {Parametrized curves in Lagrange Grassmannians},
  journal  = {Comptes Rendus Mathematique},
  year     = {2007},
  volume   = {345},
  number   = {11},
  pages    = {647--652},
  issn     = {1631-073X},
  abstract = {Curves in Lagrange Grassmannians naturally appear when one studies Jacobi equations for extremals, associated with geometric structures on manifolds. We fix integers di and consider curves Λ(t) for which at each t the derivatives of order ⩽i of all curves of vectors ℓ(t)∈Λ(t) span a subspace of dimension di. We will describe the construction of a complete system of symplectic invariants for such parametrized curves, satisfying a certain genericity assumption, and give applications to geometric structures, including sub-Riemannian and sub-Finslerian structures. To cite this article: I. Zelenko, C. Li, C. R. Acad. Sci. Paris, Ser. I 345 (2007).
Résumé
Les courbes dans les grassmanniennes lagrangiennes apparaissent naturellement lors de l'étude intrinsèque des « équations de Jacobi pour les extremas », associées à des structures géométriques sur les variétés différentielles. Nous fixons des entiers di et considérons les courbes Λ(t) pour lesquelles en chaque t les dérivées d'ordre ⩽i des ℓ(t)∈Λ(t) engendrent un sous-espace de dimension di. Nous décrirons la construction d'un système complet d'invariants symplectiques pour de telles courbes paramétrées vérifiant une condition de généricité, et nous donnerons des applications à la géométrie différentielle de structures géométriques, incluant les structures sous-riemanniennes et sous-finsleriennes. Pour citer cet article : I. Zelenko, C. Li, C. R. Acad. Sci. Paris, Ser. I 345 (2007).},
  doi      = {https://doi.org/10.1016/j.crma.2007.10.034},
  url      = {http://www.sciencedirect.com/science/article/pii/S1631073X07004347},
}

@Article{Zelenko2009,
  author   = {Igor Zelenko and Chengbo Li},
  title    = {Differential geometry of curves in Lagrange Grassmannians with given Young diagram},
  journal  = {Differential Geometry and its Applications},
  year     = {2009},
  volume   = {27},
  number   = {6},
  pages    = {723--742},
  issn     = {0926-2245},
  abstract = {Curves in Lagrange Grassmannians appear naturally in the intrinsic study of geometric structures on manifolds. By a smooth geometric structure on a manifold we mean any submanifold of its tangent bundle, transversal to the fibers. One can consider the time-optimal problem naturally associated with a geometric structure. The Pontryagin extremals of this optimal problem are integral curves of certain Hamiltonian system in the cotangent bundle. The dynamics of the fibers of the cotangent bundle w.r.t. this system along an extremal is described by certain curve in a Lagrange Grassmannian, called Jacobi curve of the extremal. Any symplectic invariant of the Jacobi curves produces the invariant of the original geometric structure. The basic characteristic of a curve in a Lagrange Grassmannian is its Young diagram. The number of boxes in its kth column is equal to the rank of the kth derivative of the curve (which is an appropriately defined linear mapping) at a generic point. We will describe the construction of the complete system of symplectic invariants for parameterized curves in a Lagrange Grassmannian with given Young diagram. It allows to develop in a unified way local differential geometry of very wide classes of geometric structures on manifolds, including both classical geometric structures such as Riemannian and Finslerian structures and less classical ones such as sub-Riemannian and sub-Finslerian structures, defined on nonholonomic distributions.},
  doi      = {https://doi.org/10.1016/j.difgeo.2009.07.002},
  keywords = {Curves in Lagrange Grassmannians, Moving frames, Young diagrams, Sub-Riemannian structures, Symplectic invariants, Quivers},
  url      = {http://www.sciencedirect.com/science/article/pii/S0926224509000710},
}

@Article{Agrachev2009,
  author   = {Agrachev, A. A.},
  title    = {Any sub-Riemannian metric has points of smoothness},
  journal  = {Doklady Mathematics},
  year     = {2009},
  volume   = {79},
  number   = {1},
  pages    = {45--47},
  month    = {Feb},
  issn     = {1531-8362},
  abstract = {We prove the result stated in the title that is equivalent to the existence of a regular point of the sub-Riemannian exponential mapping. In the case of a complete real-analytic sub-Riemannian manifold, we prove that the metric is analytic on an open everywhere dense subset.},
  day      = {01},
  doi      = {10.1134/S106456240901013X},
  url      = {https://doi.org/10.1134/S106456240901013X},
}

@Article{Weyl1921,
  author  = {H. Weyl},
  title   = {Zur Infinitisimalgeometrie: Einordnung der projektiven und der konformen Auffasung},
  journal = {Nachrichten von der K. Gesellschaft der Wissenschaften zu G\"ottingen, Mathematisch-Physikalische Klasse},
  year    = {1921},
}

@Article{Bianchini1990,
  author  = {Bianchini, R. and Stefani, G.},
  journal = {SIAM Journal on Control and Optimization},
  title   = {Graded Approximations and Controllability Along a Trajectory},
  year    = {1990},
  number  = {4},
  pages   = {903-924},
  volume  = {28},
  doi     = {10.1137/0328050},
  eprint  = {https://doi.org/10.1137/0328050},
  url     = {https://doi.org/10.1137/0328050},
}

@Article{Paoli2017,
  author   = {Paoli, Elisa},
  journal  = {Journal of Dynamical and Control Systems},
  title    = {Small Time Asymptotics on the Diagonal for H{\"o}rmander's Type Hypoelliptic Operators},
  year     = {2017},
  issn     = {1573-8698},
  month    = {Jan},
  number   = {1},
  pages    = {111--143},
  volume   = {23},
  abstract = {We compute the small time asymptotics of the fundamental solution of H{\"o}rmander's type hypoelliptic operators with drift, on the diagonal at a point x                        0. We show that the order of the asymptotics depends on the controllability of an associated control problem and of its approximating system. If the control problem of the approximating system is controllable at x                        0, then so is also the original control problem, and in this case we show that the fundamental solution blows up as                                                                                                                                                                       t                                                                          −                          N                          /                          2                                                                                                      {\$}{\backslash}phantom {\{}{\backslash}dot {\{}i{\}}{\backslash}!{\}}t^{\{}-{\backslash}mathcal {\{}N{\}}/2{\}}{\$}                , where                                                                                                                     N                                                        {\$}{\backslash}phantom {\{}{\backslash}dot {\{}i{\}}{\backslash}!{\}}{\backslash}mathcal {\{}N{\}}{\$}                 is a number determined by the Lie algebra at x                        0 of the fields, that define the hypoelliptic operator.},
  day      = {01},
  doi      = {10.1007/s10883-016-9321-z},
  groups   = {[Sofya:]},
  url      = {https://doi.org/10.1007/s10883-016-9321-z},
}

@Article{Jean2018s,
  author  = {Jean, Fr\'{e}d\'{e}ric and Maslovskaya, Sofya},
  title   = {Inverse Optimal Control Problem: The Linear-Quadratic Case},
  journal = {HAL preprint hal-01740438},
  year    = {2018},
  url     = {https://hal-ensta.archives-ouvertes.fr/hal-01740438/document},
}

@Book{Gantmacher2000,
  title     = {The Theory of Matrices.},
  publisher = {American Mathematical Society},
  year      = {1959},
  author    = {Gantmacher, F.},
  volume    = {2},
}

@Article{El-Alaoui1996,
  author   = {El-Alaoui, El-H. Ch. and Gauthier, J. -P. and Kupka, I.},
  journal  = {Journal of Dynamical and Control Systems},
  title    = {Small sub-Riemannian balls on R3},
  year     = {1996},
  issn     = {1573-8698},
  month    = {Jul},
  number   = {3},
  pages    = {359--421},
  volume   = {2},
  abstract = {This paper deals with sub-Riemannian metrics onR3 in the contact case. We study the singularities of the exponential mapping in the neighborhood of its pole. This is in stark contrast with the Riemannian case where this situation never occurs.},
  day      = {01},
  doi      = {10.1007/BF02269424},
  groups   = {Sofya:6},
  url      = {https://doi.org/10.1007/BF02269424},
}

@Article{Jameson1973,
  author    = {Antony Jameson and Eliezer Kreindler},
  journal   = {SIAM Journal on Control},
  title     = {Inverse Problem of Linear Optimal Control},
  year      = {1973},
  number    = {1},
  pages     = {1-19},
  volume    = {11},
  doi       = {10.1137/0311001},
  eprint    = {https://doi.org/10.1137/0311001},
  file      = {:Inverse\\jameson_kreindler_73.pdf:PDF},
  keywords  = {inverse problem, linear control, quadratic cost},
  owner     = {Frédéric Jean},
  timestamp = {19.03.2018},
  url       = {https://doi.org/10.1137/0311001},
}

@BOOK{Coron2007,
  title = {Control and nonlinearity},
  publisher = {American Mathematical Society},
  year = {2007},
  author = {Coron, Jean-Michel},
  volume = {136},
  pages = {xiv+426},
  series = {Mathematical Surveys and Monographs},
  address = {Providence, RI},
  file = {:Livres/coron-book.pdf:PDF},
  isbn = {978-0-8218-3668-2; 0-8218-3668-4},
  keywords = {automatic control, controle des EDP, geometric control},
  mrclass = {93-02 (35Q30 35Q53 35Q55 93C20)},
  mrnumber = {2302744 (2008d:93001)},
  mrreviewer = {Vilmos Komornik},
  owner = {Frédéric Jean},
  timestamp = {14.06.2012}
}

@Book{Bryson1975,
  title =     {Applied optimal control},
  publisher = {Hemisphere Publishing Corp. Washington, D. C.; distributed by Halsted Press [John Wiley \& Sons], New York-London-Sydney},
  year =      {1975},
  author =    {Bryson, Jr., Arthur E. and Ho, Yu Chi},
  note =      {Optimization, estimation, and control, Revised printing},
  file =      {:Livres\\Djvu\\Bryson,_Yu-Chi_Ho_Applied_Optimal.djvu:Djvu},
  keywords =  {automatic control, optimal control},
  mrclass =   {93CXX (93E10 90D25)},
  mrnumber =  {0446628},
  owner =     {Frédéric Jean},
  pages =     {xiv+481},
  timestamp = {30.03.2018}
}

@InProceedings{Liebscher1998,
  author    = {Liebscher, Dirk},
  booktitle = {Variational Calculus, Optimal Control and Applications},
  title     = {Strong Observability of Time-Dependent Linear Systems},
  year      = {1998},
  address   = {Basel},
  editor    = {Schmidt, Werner H. and Heier, Knut and Bittner, Leonhard and Bulirsch, Roland},
  pages     = {175--182},
  publisher = {Birkh{\"a}user Basel},
  abstract  = {There are considered time-dependent linear systems of the form with state x ∈ IRn, control (input) u ∈ IRmand output y ∈ IRp. We derive local characterizations of observability of (A, C) and strong observability of (A, B, C). These criteria are pointwise rank conditions on a certain matrix, which is explicitly built up from the first n --- 2 derivatives of A and B and the first n --- 1 derivatives of C. The results generalize well-known theorems for time-invariant systems.},
  file      = {:Controle/liebscher98.pdf:PDF},
  isbn      = {978-3-0348-8802-8},
  keywords  = {linear control, observer},
}

@InProceedings{Jean2018a,
  author =    {F. {Jean} and S. {Maslovskaya}},
  title =     {Inverse optimal control problem: the linear-quadratic case},
  booktitle = {2018 IEEE Conference on Decision and Control (CDC)},
  year =      {2018},
  pages =     {888-893},
  month =     {Dec},
  doi =       {10.1109/CDC.2018.8619204},
  issn =      {2576-2370},
  keywords =  {inverse problems;linear quadratic control;optimisation;inverse optimal control problem;finite horizon linear-quadratic problem;linear-quadratic case;optimality principle;cost reconstruction algorithm;Optimal control;Inverse problems;Trajectory;Symmetric matrices;Reconstruction algorithms;Cost function},
  owner =     {Frédéric Jean},
  timestamp = {14.03.2019}
}

@Book{Anderson1990,
  title =     {Optimal Control: Linear Quadratic Methods},
  publisher = {Prentice-Hall, Inc.},
  year =      {1990},
  author =    {Anderson, Brian D. O. and Moore, John B.},
  address =   {Upper Saddle River, NJ, USA},
  file =      {:Livres\\anderson_moore.PDF:PDF},
  isbn =      {0-13-638560-5},
  keywords =  {automatic control, optimal control, linear control, filtering},
  owner =     {Frédéric Jean},
  timestamp = {01.07.2015}
}

@Article{Jean2019,
  author =    {Jean, Fr{\'e}d{\'e}ric and Maslovskaya, Sofya and Zelenko, Igor},
  title =     {On projective and affine equivalence of sub-Riemannian metrics},
  journal =   {Geometriae Dedicata},
  year =      {2019},
  month =     {Mar},
  abstract =  {Consider a smooth connected manifold M equipped with a bracket generating distribution D. Two sub-Riemannian metrics on (M,Â D) are said to be projectively (resp. affinely) equivalent if they have the same geodesics up to reparameterization (resp. up to affine reparameterization). A sub-Riemannian metric g is called rigid (resp. conformally rigid) with respect to projective/affine equivalence, if any sub-Riemannian metric which is projectively/affinely equivalent to g is constantly proportional to g (resp. conformal to g). In the Riemannian case the local classification of projectively (resp. affinely) equivalent metrics was done in the classical work (Levi-Civita in Ann Mat Ser 2a 24:255--300, 1896; resp. Eisenhart in Trans Am Math Soc 25(2):297--306, 1923). In particular, a Riemannian metric which is not rigid with respect to one of the above equivalences satisfies the following two special properties: its geodesic flow possesses a collection of nontrivial integrals of special type and the metric induces certain canonical product structure on the ambient manifold. The only proper sub-Riemannian cases to which these classification results were extended so far are sub-Riemannian metrics on contact and quasi-contact distributions (Zelenko in J Math Sci (NY) 135(4):3168--3194, 2006). The general goal is to extend these results to arbitrary sub-Riemannian manifolds. In this article we establish two types of results toward this goal: if a sub-Riemannian metric is not conformally rigid with respect to the projective equivalence, then, first, its flow of normal extremals has at least one nontrivial integral quadratic on the fibers of the cotangent bundle and, second, the nilpotent approximation of the underlying distribution at any point admits a product structure. As a consequence we obtain two types of genericity results for rigidity: first, we show that a generic sub-Riemannian metric on a fixed pair (M,Â D) is conformally rigid with respect to projective equivalence. Second, we prove that, except for special pairs (m,Â n), for a generic distribution D of rank m on an n-dimensional manifold, every sub-Riemannian metric on D is conformally rigid with respect to the projective equivalence. For the affine equivalence in both genericity results conformal rigidity can be replaced by usual rigidity.},
  day =       {16},
  doi =       {10.1007/s10711-019-00437-1},
  issn =      {1572-9168},
  owner =     {Frédéric Jean},
  timestamp = {17.03.2019},
  url =       {https://doi.org/10.1007/s10711-019-00437-1}
}

@InProceedings{Jean2019a,
  author    = {Jean, Frédéric and Maslovskaya, Sofya},
  booktitle = {2019 IEEE 58th Conference on Decision and Control (CDC)},
  title     = {Injectivity of the inverse optimal control problem for control-affine systems},
  year      = {2019},
  pages     = {511-516},
  doi       = {10.1109/CDC40024.2019.9028877},
}

@Book{Kato1995,
  author    = {Kato, Tosio},
  publisher = {Springer-Verlag, Berlin},
  title     = {Perturbation theory for linear operators},
  year      = {1995},
  isbn      = {3-540-58661-X},
  note      = {Reprint of the 1980 edition},
  series    = {Classics in Mathematics},
  doi       = {10.1007/978-3-642-66282-9},
  file      = {:Livres/kato.pdf:PDF},
  mrclass   = {47A55 (46-00 47-00)},
  mrnumber  = {1335452},
  pages     = {xxii+619},
}

@Book{Lee1967,
  author    = {E.B. Lee and L. Markus},
  publisher = {Wiley, New York},
  title     = {Foundations of Optimal Control Theory},
  year      = {1967},
  file      = {:Livres/E. B. Lee, L. Markus - Foundations of Optimal Control Theory-Krieger Pub Co (1986).djvu:Djvu},
  keywords  = {optimal control},
  owner     = {Frédéric Jean},
  timestamp = {28.05.2010},
}

@PhdThesis{Maslovskaya2018,
  author      = {Maslovskaya, Sofya},
  title       = {{Inverse Optimal Control : theoretical study}},
  school      = {{Universit{\'e} Paris-Saclay}},
  year        = {2018},
  type        = {Theses},
  month       = Oct,
  file        = {72687_MASLOVSKAYA_2018_archivage.pdf:https\://pastel.archives-ouvertes.fr/tel-01950176/file/72687_MASLOVSKAYA_2018_archivage.pdf:PDF},
  hal_id      = {tel-01950176},
  hal_version = {v1},
  keywords    = {Neurophysiology ; Geometric control ; Optimal control ; Neurophysiologie ; Contr{\^o}le g{\'e}om{\'e}trique ; Contr{\^o}le optimal},
  number      = {2018SACLY013},
  url         = {https://pastel.archives-ouvertes.fr/tel-01950176},
}

@Article{Bonnard2018,
  author      = {Bonnard, Bernard and Chyba, Monique and Rouot, J{\'e}r{\'e}my and Takagi, Daisuke},
  journal     = {{Pacific Journal of Mathematics for Industry}},
  title       = {Sub-Riemannian geometry, Hamiltonian dynamics, micro-swimmers, Copepod nauplii and Copepod robot},
  year        = {2018},
  month       = Dec,
  number      = {2},
  volume      = {10},
  doi         = {10.1186/s40736-018-0036-9},
  file        = {:Nageurs\\bonnard_survey-nageurs_2017.pdf:PDF;survey-nageurs.pdf:https\://hal.archives-ouvertes.fr/hal-01653901/file/survey-nageurs.pdf:PDF},
  hal_id      = {hal-01653901},
  hal_version = {v1},
  keywords    = {Optimality conditions ; Direct and indirect numerical methods in optimal control ; Geometric optimal control ; Sub-Riemannian geometry ; Micro-swimmers and efficient strokes ; Closed geodesics in Riemannian geometry, swimmer},
  owner       = {Frédéric Jean},
  publisher   = {{Springer}},
  timestamp   = {20.12.2017},
  url         = {https://hal.archives-ouvertes.fr/hal-01653901},
}






@Article{Giraldi2020,
  author   = {Giraldi, Laetitia and Jean, Fr\'{e}d\'{e}ric},
  journal  = {SIAM Journal on Control and Optimization},
  title    = {Periodical Body Deformations are Optimal Strategies for Locomotion},
  year     = {2020},
  number   = {3},
  pages    = {1700-1714},
  volume   = {58},
  abstract = {A periodical cycle of body deformation is a common strategy for locomotion (see, for instance, birds, fishes, humans). The aim of this paper is to establish that the autopropulsion of deformable objects is optimally achieved using periodic strategies of body deformations. This property is proved for a simple model using an optimal control theory framework.},
  doi      = {10.1137/19M1280120},
  eprint   = {https://doi.org/10.1137/19M1280120},
  url      = {https://doi.org/10.1137/19M1280120},
}

@Article{Bettiol2019,
  author  = {{Bettiol, P.} and {Bonnard, B.} and {Nolot, A.} and {Rouot, J.}},
  journal = {ESAIM: COCV},
  title   = {Sub-Riemannian geometry and swimming at low Reynolds number: the Copepod case},
  year    = {2019},
  pages   = {9},
  volume  = {25},
  doi     = {10.1051/cocv/2017071},
  url     = {https://doi.org/10.1051/cocv/2017071},
}

@Book{Alexander1997,
  author      = {R. McNeill Alexander},
  publisher   = {Princeton University Press},
  title       = {Optima for Animals},
  year        = {1997},
  address     = {Princeton},
  isbn        = {9780691221601},
  doi         = {doi:10.1515/9780691221601},
  lastchecked = {2024-06-18},
  url         = {https://doi.org/10.1515/9780691221601},
}

@Article{McFarland1977,
  author   = {McFarland, D. J.},
  journal  = {Nature},
  title    = {Decision making in animals},
  year     = {1977},
  issn     = {1476-4687},
  number   = {5623},
  pages    = {15--21},
  volume   = {269},
  abstract = {Animals must make decisions about when to feed, when to court, when to sleep, and so on, in such a way as to maximise as far as possible their chances of survival and reproductive success. It is possible to formulate in mathematical terms the optimal strategy for an animal to pursue. The theoretical optimum behaviour can be compared with the actual behaviour of the animal, and perhaps shed some light on the evolution of behaviour.},
  doi      = {10.1038/269015a0},
  refid    = {McFarland1977},
  url      = {https://doi.org/10.1038/269015a0},
}

@Article{Westermann2020,
  author   = {Westermann, Kevin and Lin, Jonathan Feng-Shun and Kulić, Dana},
  journal  = {Scientific Reports},
  title    = {Inverse optimal control with time-varying objectives: application to human jumping movement analysis},
  year     = {2020},
  issn     = {2045-2322},
  number   = {1},
  pages    = {11174},
  volume   = {10},
  abstract = {Analysis of complex human movements can provide valuable insights for movement rehabilitation, sports training, humanoid robot design and control, and human-robot interaction. To accomplish complex movement, the central nervous system must coordinate the musculo-skeletal system to achieve task and internal (e.g., effort minimisation) objectives. This paper proposes an inverse optimal control approach for analysing complex human movement that does not assume that the control objective(s) remains constant throughout the movement. The movement trajectory is assumed to be optimal with respect to a cost function composed of the sum of weighted basis cost functions, which may be time varying. The weights of the cost function are recovered using a sliding window. To illustrate the proposed approach, a dataset consisting of standing broad jump to targets at three different distances is collected. The method can be used to extract control objectives that influence task success, identify different motion strategies/styles, as well as to observe how control strategy changes during the motor learning process. Kinematic analysis confirms that the identified control objectives, including centre-of-mass takeoff vector and foot placement upon landing are important to ensure that a given participant lands on the target. The dataset, including nearly 800 jump trajectories from 22 participants is also provided.},
  doi      = {10.1038/s41598-020-67901-x},
  refid    = {Westermann2020},
  url      = {https://doi.org/10.1038/s41598-020-67901-x},
}

@Comment{jabref-meta: databaseType:bibtex;}

